Beyond CO2 Emissions: The Overlooked Impact of Water Consumption of Information Retrieval Models

As in other fields of artificial intelligence, the information retrieval community has grown interested in investigating the power consumption associated with neural models, particularly models of search. This interest has become particularly relevant as the energy consumption of information retrieval models has risen with new neural models based on large language models, leading to an associated increase of CO2 emissions, albeit relatively low compared to fields such as natural language processing.

==> sections/results.tex <==
\subsection{Results}
\label{sec:results}





\subsubsection{Impact of Experiments on Emissions}
We begin our analysis by first investigating the emissions cost for obtaining a single result. For simplicity, we refer to the concept of an entire Information Retrieval pipeline, from training or tuning; to indexing; to retrieval or re-ranking in order to measure the effectiveness of a method, as an \textit{experiment}. These experiments on the methods described in Section~\ref{sec:experimental-setup} are presented in Table~\ref{tbl:results}.% Each stage is measured by the running time, the power consumption, and emissions.

Examining `traditional' pipelines like BM25 and learning to rank, the emissions produced by these methods is several orders of magnitude lower than more recent neural methods. This result suggests that one can perform hundreds of experiments using these methods before reaching the number of emissions produced by `modern' methods. The LTR is so close to BM25 in the number of emissions produced because it is using a linear ranker. 

A neural ranker is likely to produce more emissions. In contrast, monoBERT produces ten times more emissions to obtain a single result than other methods when comparing the neural methods. Conversely, DPR produces the least amount of emissions. As discussed below, the amount of emissions produced may be an indirect indication of effectiveness. 

Next, we further investigate the emissions produced by each neural method for an experiment. Comparing uniCOIL and TILDEv2, two document expansion models, we found that although the retrieval stage of TILDEv2 is more efficient than uniCOIL, the overall cost of an experiment is higher. Furthermore, these two methods have an expansion stage where we chose to use TILDE and docTquery. The running time of docTquery is almost 70 times that of TILDE, producing over 100 times more emissions. Across all neural methods, excluding the document expansion step, the training step was the most expensive. It produced the most emissions, with monoBERT producing approximately ten times as much during the training process as other neural methods. This is likely because monoBERT is using the \texttt{bert-large} model and because it cannot pre-compute document representations, instead needing to estimate relevance at query time. On the other hand, TILDEv2 pre-computes everything at the indexing time, costing less at retrieval time.

To get an understanding of how many emissions are produced by these methods compared to more familiar reference points, Table~\ref{tbl:appliances} contains the emissions produced by common household appliances, air travel, and car travel. Obtaining a single result for a given experiment is comparable to the emissions produced through the usage of common household appliances. A single researcher may produce the same emissions as taking a short commercial airline flight throughout model development. A research lab will naturally produce more emissions (although more difficult to estimate).\footnote{Sourcing data for Table~\ref{tbl:appliances} was challenging due to limited availability. Appliance data was sourced from ENERGY STAR (\url{https://www.energystar.gov/productfinder/advanced}). Specific URLs are listed in our repository. Flight data was sourced from \url{https://www.atmosfair.de/en/offset/flight/}. Car data was sourced from \url{https://www.epa.gov/automotive-trends/explore-automotive-trends-data}. Accessed in January 2022.}



\subsubsection{Cost of Experiment versus Cost in Production}
Research and experiments are often only one side of the coin in IR. The flip side of research is the deployment of IR systems. Using Equation~\ref{eq:query}, we plot the estimated emissions produced for each of the methods in Table~\ref{tbl:results}, presented in Figure~\ref{fig:queries}. This figure only visualises the search stage and not the entire pipeline. Furthermore, it is unlikely that a single machine will handle tens of millions of queries per hour alone; instead, a distributed system involving many servers is used for load balancing. For some systems such as monoBERT, the estimates are impossible on a single machine, as evidenced in Table~\ref{tbl:results} where only approximately 300 queries can be processed per hour (dev size/running time). Therefore the estimates offer a perspective on a likely lower bound in the emissions produced that do not consider additional resources that would be used to load-balance a production system. Additionally, the x-axis in Figure~\ref{fig:queries} only goes to 10,000,000 queries per hour. This is a low value compared to the traffic popular search engines may receive, although finding a reliable number is difficult, so our estimates are conservative.\footnote{DuckDuckGo shares official traffic statistics (\url{https://duckduckgo.com/traffic}), however they have a relatively low market share.}

Given our estimates for the number of emissions produced by a given search system, we found that even at large scales on the order of millions of queries per hour, most methods produce relatively low amounts of emissions. With our approximate, lower-bound estimates, the second worst method in terms of emissions, uniCOIL, could be run in a production system for an entire year and not produce the same amount of emissions as a flight from Melbourne to Madrid; monoBERT, on the other hand, would produce approximately the same amount in a single hour.  Finally, although TILDEv2 produces more emissions to achieve a single experimental result (as in Table~\ref{tbl:results}), in production, it is the second best behind BM25. This finding suggests that there can be a trade-off also in producing more emissions to train a model where it will produce lower emissions in production over the lifetime of the model. Note that in production systems, it is likely that query results would be cached to avoid needing to perform an end-to-end query processing pipeline. We leave such investigations for future work.



%\vspace{-4pt}
\subsubsection{Effectiveness-Emissions Trade-off}
As alluded to earlier, we observe a trade-off in the number of emissions produced for an experiment and the effectiveness that the experiment obtains. Figure~\ref{fig:tradeoff} highlights the trend that we observe for each of the methods listed in Table~\ref{tbl:results} (excluding the learning to rank experiment given the explanation in Section~\ref{sec:implementation-details}). This figure suggests that in order to achieve more effective results, more power must be used, and thus more emissions may be produced. This is particularly evident when comparing the expansion methods of TILDEv2 and uniCOIL. The docTquery expansion method results in a higher MRR@10 with a considerable trade-off in emissions.

Notably, the amount of emissions produced appears to plateau as effectiveness increases (as indicated by the blue trend line). This trend suggests that large improvements in effectiveness can be achieved when using neural methods compared to traditional methods such as BM25. However, minor improvements in effectiveness between such models come at the expense of relatively high power usage and thus emission production.




